Antenna system characteristic and solar radio burst observation

Chinese Spectral Radio Heliograph (CSRH) is an advanced aperture synthesis solar radio heliograph, developed by National Astronomical Observatories, Chinese Academy of Sciences independently. It consists of 100 reflector antennas, which are grouped into two antenna arrays (CSRH-I and CSRH-II) for low and high frequency bands respectively. The frequency band of CSRH-I is 0.4-2GHz and for CSRH-II, the frequency band is 2-15GHz. In the antenna and feed system, CSRH uses an Eleven feed to receive signals coming from the Sun, the radiation pattern with lower side lobe and back lobe of the feed is well radiated. The characteristics of gain G and antenna noise temperature T effect the quality of solar radio imaging. For CSRH, measured G is larger than 60 dBi and $ T $ is less than 120K, after CSRH-I was established, we have successfully captured a solar radio burst between 1.2-1.6GHz on November 12, 2010 through this instrument and this event was confirmed through the observation of Solar Broadband Radio Spectrometer (SBRS) at 2.84GHz and Geostationary Operational Environmental Satellite (GOES). In addition, an image obtained from CSRH-I clearly reveals the profile of the solar radio burst. The other observational work is the imaging of Fengyun-2E geosynchronous satellite which is assumed to be a point source. This data processing method indicates that, the method of deleting errors about dirty image could be used for processing other surface sources.

==> readme <==
Dear Colleagues: 

The final publication layout will be produced by using raa.cls. 
Therefore, we strongly encourage you to prepare your LaTeX manuscript 
with this class file. Please unpack raa-package.tar.gz, it includes 

raa.cls        ---- RAA macro class file for LaTeX2e 
sample.tex     ---- a sample file using raa.cls (LaTeX source) 
sample.ps      ---- the PS file created by sample.tex in referee format  
sample.pdf     ---- the PDF file created by sample.tex in referee format  
readme         ---- this file  
f?.eps         ---- three demo figures used in the LaTeX template source
sample2.tex    ---- a sample file for using raa.bst
sample2_fig?.eps -- two demo figures used in sample2.tex
sample2.pdf    ---- the PDF file created by sample.tex in referee format
sample2.bbl    ---- bibliography file using by sample2.tex
bibtex.bib     ---- an example for bibtex file

natbib.sty     ---- This package reimplements the LaTeX \cite command
natnotes.pdf   ---- Brief reference sheet for Natbib (pdf)
raa.bst        ---- Bibliography style file 

Hope you enjoy the use of this macro. Your suggestions and comments are 
highly welcome. Thanks.

Editorial Office
E-mail:  raa@raa-journal.org

